Studying the impacts of pre-training using ChatGPT-generated text on downstream tasks

In recent times, significant advancements have been witnessed in the field of language models, particularly with the emergence of Large Language Models (LLMs) that are trained on vast amounts of data extracted from internet archives. These LLMs, such as ChatGPT, have become widely accessible, allowing users to generate text for various purposes including articles, essays, jokes, and poetry. Given that LLMs are trained on a diverse range of text sources, encompassing platforms like Reddit and Twitter, it is foreseeable that future training datasets will also incorporate text generated by previous iterations of the models themselves. In light of this development, our research aims to investigate the influence of artificial text in the pre-training phase of language models. Specifically, we conducted a comparative analysis between a language model, RoBERTa, pre-trained using CNN/DailyMail news articles, and ChatGPT, which employed the same articles for its training and evaluated their performance on three downstream tasks as well as their potential gender bias, using sentiment analysis as a metric. Through a series of experiments, we demonstrate that the utilization of artificial text during pre-training does not have a significant impact on either the performance of the models in downstream tasks or their gender bias. In conclusion, our findings suggest that the inclusion of text generated by LLMs in their own pre-training process does not yield substantial effects on the subsequent performance of the models in downstream tasks or their potential gender bias.

==> sections/limitations.tex <==

\noindent While our research provides valuable insights, it is important to acknowledge the limitations inherent in our study:
\begin{enumerate}
    \item \textbf{Limited to a specific data source}: Our research focuses on a specific data source, such as the news articles from CNN/DailyMail dataset. The language models are generally trained on a much larger corpus covering variety of data sources such as books, wikipedia, social media channels like facebook, twitter and reddit. The specific data source in our study may not fully capture the diversity of domains and topics present in language model training and generation. Therefore there is risk that the limited scope may restrict the generalizability of our findings to other datasets or sources, potentially limiting the broader applicability of our results and conclusions.
    \item \textbf{Sensitivity of prompting and steering}: The generation of text by language models is highly sensitive to the prompts provided. The choice of prompts for steering data generation can influence the output and potentially introduce biases or limitations. In our study we did not explore the ability to steer the outputs of ChatGPT using different prompting. But it is possible the public users can steering the results to generate unfair, biased and unrepresentative outputs. Which may result in different outcomes on bias metrics and could be explored in future.
    \item \textbf{Language restriction to English}: Our study focuses exclusively on the English language. This limitation prevents us from examining language-specific nuances, biases, and behaviors that may differ in other languages. Expanding the analysis to include multiple languages would provide a more comprehensive understanding of the language models' performance and biases across different linguistic contexts.
    \item \textbf{Exclusive use of ChatGPT}: Our research solely utilizes the ChatGPT-0301 language model which has built in safeguards for minimising the generation of bias and harmful content. We do not study the effects of 
    uncensored language models that do not rely on human feedback for safety such as Wizard-Vicuna-30B-Uncensored-GGML\footnote{https://huggingface.co/TheBloke/Wizard-Vicuna-30B-Uncensored-GGML}. This choice limits our understanding of how different language models will effect our results and findings and may restrict the broader analysis of language generation models as a whole.
    \item \textbf{Bias Metrics}: While our research specifically explores the gender bias using a sentiment analysis task, it neglects the examination of other forms of biases, such as racial or cultural biases. Moreover there are various methods and definitions for evaluation biases in a model. These biases could be explored in future research as the language model evolves.
    
\end{enumerate}

